Flare and CME Properties and Rates at Sunspot Minimum

The corona at solar minimum generally differs greatly from that during active times. We discuss the current Cycle 23/24 minimum from the point of view of the occurrence of flares and CMEs (Coronal Mass Ejections). By comparison with the previous minimum, the flare/CME ratio diminished by almost an order of magnitude. This suggests that the environmental effect in flare/CME association differed in the sense that the Cycle 23/24 minimum corona was relatively easy to disrupt.

==> journals.tex <==
\renewcommand{\adv}{    {\rm Adv. Spa. Res.}\ }
\renewcommand{\annG}{   {\rm Annales Geophysicae}\ }
\renewcommand{\aap}{    {\rm Astron. Astrophys.}\ }
\renewcommand{\aaps}{   {\rm Astron. Astrophys. Suppl.}\ }
\renewcommand{\aapr}{   {\rm Astron. Astrophys. Rev.}\ }
\renewcommand{\ao}{     {\rm Appl. Opt.}\ }
\renewcommand{\ag}{     {\rm Ann. Geophys.}\ }
\renewcommand{\aj}{     {\rm Astronom. J.}\ }
\renewcommand{\apj}{    {\rm Astrophys. J.}\ }
\renewcommand{\apjl}{   {\rm Astrophys. J. Lett.}\ }
\renewcommand{\apjs}{   {\rm Astrophys. Suppl.}\ }
\renewcommand{\apss}{   {\rm Astrophys. Spa. Sci.}\ }
\renewcommand{\araa}{   {\rm ARAA}\ }
\renewcommand{\cjaa}{   {\rm Chinese J. Astron. Astrophys.}\ }
\renewcommand{\gafd}{   {\rm Geophys. Astrophys. Fluid Dyn.}\ }
\renewcommand{\grl}{    {\rm Geophys. Res. Lett.}\ }
\renewcommand{\ijga}{   {\rm Int. J. Geomag. Aeron.}\ }
\renewcommand{\jastp}{  {\rm J. Atmos. Sol. Terr. Phys.}\ }
\renewcommand{\jgr}{    {\rm J. Geophys. Res.}\ }
\renewcommand{\mnras}{  {\rm Mon. Not. Roy. Astron. Soc.}\ }
\renewcommand{\nat}{    {\rm Nature}\ }
\renewcommand{\pasp}{   {\rm Pub. Astron. Soc. Pac.}\ }
\renewcommand{\pasj}{   {\rm Pub. Astron. Soc. Japan}\ }
\renewcommand{\pre}{    {\rm Phys. Rev. E}\ }
\renewcommand{\solphys}{{\rm Solar Phys.}\ }
\renewcommand{\sovast}{ {\rm Sov. Astronom.}\ }
\renewcommand{\ssr}{    {\rm Space Sci. Rev.}\ }


